Rethinking Traffic Flow Forecasting: From Transition to Generatation

Traffic flow prediction plays an important role in Intelligent Transportation Systems in traffic management and urban planning. There have been extensive successful works in this area. However, these approaches focus only on modelling the flow transition and ignore the flow generation process, which manifests itself in two ways: (i) The models are based on Markovian assumptions, ignoring the multi-periodicity of the flow generation in nodes. (ii) The same structure is designed to encode both the transition and generation processes, ignoring the differences between them. To address these problems, we propose an Effective Multi-Branch Similarity Transformer for Traffic Flow Prediction, namely EMBSFormer. Through data analysis, we find that the factors affecting traffic flow include node-level traffic generation and graph-level traffic transition, which describe the multi-periodicity and interaction pattern of nodes, respectively. Specifically, to capture traffic generation patterns, we propose a similarity analysis module that supports multi-branch encoding to dynamically expand significant cycles. For traffic transition, we employ a temporal and spatial self-attention mechanism to maintain global node interactions, and use GNN and time conv to model local node interactions, respectively. Model performance is evaluated on three real-world datasets on both long-term and short-term prediction tasks. Experimental results show that EMBSFormer outperforms baselines on both tasks. Moreover, compared to models based on flow transition modelling (e.g. GMAN, 513k), the variant of EMBSFormer(93K) only uses 18\% of the parameters, achieving the same performance.

==> checklist.tex <==
# abs ok
# intro 补充 生成和转移过程的描述
# 

==> introduction.tex <==
\begin{abstract}
交通流预测在交通管理领域起到重要作用。其中，捕捉周期性与趋势性是交通流预测中的重要挑战。目前自注意力机制和GNN是解决该问题最有效的方法之一，然而基于它们建立的模型存在以下两点限制。（i）目前绝大多数的交通流预测模型都是基于马尔可夫假设，它们没有考虑到多周期的影响。(ii) 现有主流方法对周期性和趋势性采用相同的结构进行编码，忽略了两种信号的差异，限制了模型的表示能力。为解决以上挑战，我们提出ASTGFormer进行交通流预测。通过数据分析我们发现，影响趋势性和周期性的因素不同，所以我们将问题分为多周期性和趋势性分别应对：(i) 对多周期，通过相似分析模块结构充分利用多周期性，并支持多轮模式周期的引入，以适应更多周期性的数据 (ii) 对趋势性（邻近性），通过时间自注意力机制对时间信息聚类，空间自注意力机制对空间信息聚类，GNN分析交通流量的流通性。我们通过大量实验证明方法高效性与有效性，模型在实验中表现优异，分别在长程预测优于MAE(), MAPE(), RMSE()，短程预测优于MAE(), MAPE(), RMSE()。并且，相比于以注意力机制为基础的模型，仅采用\20\%参数的相似模块能达到与众多模型同样性能。
\end{abstract}


\begin{introduction}
日益增加的出行需求加剧了交通拥堵，高准确率的交通流预测在智慧交通管理系统多个应用领域上起到非常重要的作用，如车辆调度，路线规划，缓解拥堵等。一直以来，交通流预测受到趋势性和周期性的重要挑战。

在一方面，如图(a)(b)所示，具有邻接关系的Node A 和 Node B, 在日常流量和突发情况表现出极为相似的走势，而不具备直接邻接关系的Node C没有相似特点。另一方面，交通流周期性则体现点位的通用特性，如图(c)(d)所示，历史流量分别在以天，周表现出周期性。由图分析，两个特征表现出交通流量的不同影响，其中趋势性更多体现在交通特殊情况，如交通拥堵，交通事故等。周期性更多体现在当前时间点位的总体流量。

（背景介绍 图(a) 点位在地图展示 图描述 图(b) 展现交通流量趋势性   图(c) ying展现交通流量周期性-天  图(d) 展现交通流量周期性-周 图(e) 展现假期对交通流量的影响）

近年来深度学习方法极大地促进了交通流预测的发展。卷积神经CNNs与RNNs首先用于应对基于网格的流量预测(ST-ResNet, DMVST-Net),GNNs方法的引入学习交通趋势性(STGCN, ASTGCN), 之后，注意力机制的引入促进空间，时序数据的信息聚合和挖掘(STTN,ASTGNN,SSTBAN)。尽管基于GNNs和自注意力机制的模型能够较好地应对趋势性和周期性，然而它们依然存在以下限制。

(i) 大多数模型并没有考虑交通流的多周期性。大多数序列到序列的预测是一个遵循马尔可夫假设的任务，基于马尔科夫假设进行建模的模型仅考虑了临近的前序节点对预测的影响，但是交通流受到长程历史的影响，如图1(c)(d)所示, 交通历史流量分别表现出以天，周为周期的多周期性，这说明交通流量在短程时序分析外，还需考虑长周期性的影响。 

(ii) 少数考虑长周期性的模型并没有高效地解决它。例如，ASTGCN，AGCAN（2021）考虑了长周期性的影响，将数据分为长期历史与短期历史分别应对趋势性与长周期性，但是，它们忽略了趋势性与周期性的信号特征差异，如图（c）(d)(e)所示，采用相同的学习结构编码分别应对趋势性和周期性，为分析多周期性引入了多余的噪声信息，这不仅没有有效地解决的多周期性，还为模型增加了训练负担。

为解决上述挑战，在这篇文章，我们提出基于长短历史相似性引导的图卷积转换器网络ASTGFormer进行交通流预测。我们将问题拆分为解决趋势性和多周期性，分别在近期历史与长期历史解决。首先，通过数据嵌入模块嵌入多源特征，以供训练。在一方面，我们采用近期模块来应对趋势性，以自注意力为基础分别在空间和时间上进行数据聚类，通过图卷积引入空间邻接信息，分析流量趋势性。 另一方面，我们提出相似模块专门应对长周期性，模块中，提出相似注意力机制仅分析近期与长期历史的相似关系，大大减轻了训练负荷。最后通过模块获得预测结果。综上所述，本片文章主要贡献如下：

\begin{itemize}
    \item 归纳区分邻接性和长周期性重要挑战, 并提出基于历史相似性引导的图卷积转换器模型ASTGFormer分别应对趋势性和长周期性，出色完成交通流预测。

    \item 我们设计近期模块和相似分别分析模块分析趋势性和长周期性，在相似分析模块，提出相似注意力机制，高效地解决了周期性的问题，并为近期模块提供了引导作用。

    \item 我们在4个数据集对模型分别进行了短序列和长序列预测的实验。结果表现出我们模型在短序列预测最高优于模型（），长序列预测最高优于模型（），并且，消融，可视化实验与性能分析充分展现了模型的高效性和有效性。
\end{itemize}
\end{introduction}
